Moving-Horizon State Estimation for Power Networks and Synchronous Generators

Power network and generators state estimation are usually tackled as separate problems. We propose a dynamic scheme for the simultaneous estimation of the network and the generator states. The estimation is formulated as an optimization problem on a moving-horizon of past observations. The framework is a generalization of static state estimation; it can handle incomplete model knowledge and does not require static network observability by PMUs. The numerical results show an improved estimation accuracy compared to static state estimation. Moreover, accurate estimation of the internal states of generators without PMUs on their terminals can be achieved. Finally, we highlight the capability of the proposed estimator to detect and identify bad data.

==> test.tex <==
therefore power system is modelled with a set of differential-algebraic equations (DAE) of index 1
\begin{subequations}
\begin{align}
    \dot{x}& = f(x, u, p),\\
    0 &= g(x, u, p).
\end{align}
\end{subequations}

Integration of power electronics-interfaced generation into the estimation scheme will be addressed in future work. 
where $x$ represents differential states of generators, $u$ algebraic states, i.e. nodal voltages, and $p$ represents a set of parameters of interest. 

PMUs are being deployed in power systems around the world, but still, most of the networks are not observable using PMU data only. This lack of observability represents  a challenge for the implementation of fast, real-time state estimation.


Finally, our approach can detect bad data Leveraging dynamic equations to detect bad data and cyber-attacks has been recognized in the literature. However, the   \par

 However, the effect of bad data in the measurement set was not analyzed. In \cite{DSE_cs1}, the authors designed a dynamic estimator based on the EKF, robust against cyber-attacks. They used the second-order swing equation generator model, which requires knowledge of the transient internal voltage for initializing the estimation. However, in the case of bad data in the measurements, reliable estimation of this internal voltage cannot be guaranteed. Cyber-attacks on DSE were also reported in \cite{DSE_cs2}, \cite{DSE_cs3}. However, the assumption was that each generator node is equipped with a PMU device. In this work, we show that it is possible to detect bad data in the measurements,  \par
 
 Our approach does not require access to the generator PMUs nor does it require the network observability by PMU measurements. \par
